Image-Space Collage and Packing with Differentiable Rendering

Collage and packing techniques are widely used to organize geometric shapes into cohesive visual representations, facilitating the representation of visual features holistically, as seen in image collages and word clouds. Traditional methods often rely on object-space optimization, requiring intricate geometric descriptors and energy functions to handle complex shapes. In this paper, we introduce a versatile image-space collage technique. Leveraging a differentiable renderer, our method effectively optimizes the object layout with image-space losses, bringing the benefit of fixed complexity and easy accommodation of various shapes. Applying a hierarchical resolution strategy in image space, our method efficiently optimizes the collage with fast convergence, large coarse steps first and then small precise steps. The diverse visual expressiveness of our approach is demonstrated through various examples. Experimental results show that our method achieves an order-of-magnitude speedup compared to state-of-the-art techniques. The project page is https://szuviz.github.io/pixel-space-collage-technique/.

==> tex/5_discussion.tex <==
\section{Discussion}

In this section, we delve into the limitations of our method, addressing areas where improvements can be made. 

\textbf{Filling Quality} In our experiment, we discovered that when visual primitives are not limited by data encoding fidelity, we can achieve high-quality filling results. This means that the filling, as shown in Figure~\ref{fig:word_pack} with the example of wine, has minimal overlap and is compact. However, when we introduce data fidelity constraints, there may be some overlapping among visual primitives, as observed in the US map depicted in Figure~\ref{fig:teaser}. In such cases, our filling quality may not be as good as that achieved by specialized tools like \textit{ShapeWordle}~\cite{wang2019shapewordle} in wordle. Additionally, the filling quality of icons is inferior to that of specialized geometric descriptors~\cite{kwan2016pyramid}. Hence, for future research, a promising approach would involve combining image-space collage techniques as a solid foundation, supplemented by a few optimization steps in the object-space to enhance the filling rate. This combined methodology has the potential to yield significant improvements in achieving a satisfactory filling outcome.

\textbf{Shadow Trap} During the optimization process, it is possible to encounter situations where a primitive becomes immobilized due to being fully obstructed or covered by other primitives. As depicted in Figure~\ref{fig:shadowtrap}, some small primitives are surrounded, rendering them unable to freely adjust and fit into their surroundings. This obstruction leads to a state of stagnation, where the primitive remains stationary and unable to move. To address this issue, a potential solution for overcoming the "shadow trap" could involve implementing intelligent algorithms that detect and prevent the complete coverage of primitives. By incorporating adaptive strategies or dynamic rearrangement techniques, future research could aim to enhance the object's ability to navigate its surroundings and avoid getting trapped. This avenue of investigation holds promise for improving the overall optimization process and achieving more desirable results.

\begin{figure}[!htb]
  \centering
    \includegraphics[width=.95\linewidth]{fig/shadowtrap.png}
    % {img/match.png}
    \caption{Shadow Trap in Optimization: primitive becomes immobilized due to being fully obstructed or covered by other primitives.}
  \label{fig:shadowtrap}
\end{figure}

\textbf{Primitive Seeding} In this study, we experimented with a MAT-based method for assigning primitives by considering their sizes and placing them along median axes. This approach proves highly effective for shapes with varying widths, including tubes and necks, as seen in the shape `@' and `tail of seahorse' in Figure~\ref{fig:word_pack}. Our experiments validate the promising results achieved through this initialization technique. However, it is important to note while our MAT-based method succeeds for certain shapes, it may not be optimal for others. For instance, when dealing with round bellies, an alternative approach like random sampling can be more suitable and effective. A well-chosen initialization contributes significantly to accurate and efficient shape representation. Therefore, we strongly encourage further research efforts to develop intelligent seeding techniques that automatically suggest or generate initial visual primitives based on the underlying data characteristics. This would streamline the visualization creation process and provide users with a starting point for their designs.


==> tex/5_link2model.tex <==
% \section{Linked with Generative Models}

% Text2image model, prompting engineering, mask, 

% Our image-space collage technique can incorporate the use of image generative models as a source for the target image. This means that the process is not limited to using pre-existing images as targets. For example, users can input text instead of an image. The text is then processed through an image generative model to produce a corresponding visual output. This output then serves as the target image for the collage visualization process. The technique thus allows for the generation of collage visualizations from textual inputs.



==> tex/6_evaluation_old.tex <==
\section{Evaluation}

%\lmc{to be shortened}
%In this section, we present our method's capabilities in data visualizations across a wide range of examples, including conventional visualizations (Section~\ref{subsec:convvis}) and infographic visualization (Section~\ref{subsec:illustr}) \lmc{to be changed}. \lm{In the examples where force attraction loss is used, e.g., the Nobel example in Figure~\ref{fig:nobel}, we showed the attracting force by a green arrow. Other examples without force attraction are generated using the combination of three loss functions, including boundary fitness, primitive overlap, and even distribution.}

In this section, we first report the results of the ablation study and then elaborate on the comparison between our method and three state-of-the-art methods.  

\paragraph{Metrics of Collage Quality} We used five metrics to quantitatively measure the quality of the generated collages. The first three metrics are adopted from exiting work~\cite{wang2019shapewordle}, and additional two metrics are added to quantify the overlaps among objects and the target shape: 
(1) \textit{Layout Coverage (LC):} it is quantified as the proportion between the number of pixels in the object area (i.e., words in the clouds) and the number of pixels in the non-object area inside the target shape, the bigger the better; (2) \textit{Layout Uniformity (LU)}: \lmn{it is quantified as the reciprocal of the averaged distance square of non-object pixels in the target shape to the nearest objects}, the larger the better; (3) \textit{Shape Alignment (SA)}: \lmn{it is quantified as the reciprocal of the averaged squared distance of pixels on the shape contour to the nearest objects.} A larger value indicates better shape alignment. 
%it is quantified as the averaged distance square of pixels on the shape contour to the nearest objects, the smaller the better; 
(4) \textit{Object Overlap (OO)}: it is quantified as the ratio of pixels in the overlap areas between objects to the total number of pixels in the target shape; (5) \textit{Exceeding Area (EA):} it is quantified as the ratio of pixels that exceed the target shape to the total number of pixels in the target shape. 

% \subsection{Examples}

% \textbf{}

% In the first user study on computational efficiency, we measured the time consumption of our technique. In the second study on data encoding fidelity, we examined how well our method preserves the original data throughout the collage creation process.

\subsection{Ablation Study} 
\label{subsec:ablation}

\paragraph{Ablation on Uniform Loss} We investigated the impact of uniform loss on collage quality. As shown in Figure~\ref{fig:uniform}, \textit{without the uniform loss}, the elements are less evenly distributed. For example, in the highlighted regions, collages without uniform loss leave noticeable gaps in other areas, which disrupts the overall balance and aesthetic consistency of the design.


\begin{figure}[!htb]
  \centering
    \includegraphics[width=1.\linewidth]{fig/uniform2.png}
    % {img/match.png}
    \caption{Comparison of collages with and without the uniform loss: with uniform loss, the elements (e.g., texts on the right example) exhibit a more evenly distributed arrangement.}
  \label{fig:uniform}
\end{figure}


\paragraph{Ablation on Hierarchical Image Resolution} We conducted an ablation study to evaluate the impact of different image resolution strategies on performance. The study examined six resolution approaches: constant $200 \times 200$, constant $400 \times 400$, constant $600 \times 600$ and $800 \times 800$, hierarchical resolutions 200 + 800, and hierarchical resolutions 200 + 500 + 800. 

The evaluation was performed under four experimental conditions, defined by varying the number of geometric elements (100, 300) and two collage shapes. These conditions allowed us to assess how the resolution strategies performed under different design complexities. The results, summarized in Figure~\ref{}\lmc{tba}, reveal clear trade-offs between resolution strategy and time cost. The constant high-resolution approaches (Constant $300 \times 300$ and Constant $500 \times 500$) achieved high metric scores but incurred significant computational overhead. In contrast, the hierarchical strategies, especially 100 + 300 and 100 + 300 + 500, demonstrated more balanced performance. They delivered competitive metric results while maintaining lower time costs, highlighting their efficiency in managing resolution adaptively.


\subsection{Comparison Experiment}

We compared our method with three existing techniques, ShapeWordle~\cite{wang2019shapewordle}, PAD~\cite{kwan2016pyramid}, and ShapeCollage~\cite{shapecollage}. These methods are limited to specific types of geometric objects: ShapeWordle for texts, PAD for shapes, and ShapeCollage for images. Since their generalizability to other geometric types is not straightforward, we performed a one-on-one comparison between our method and these baselines. 

%Except for ShapeWordle used for text data visualization, the direct use of PAD and ShapeCollage to encode data is unclear. 

\iffalse
\begin{table}[!htb]
\centering
\caption{Overview of three baselines and our method.}
\label{table:brief}
\begin{tabular}{c|c|c}
      Method       & Collage of General Objects &  Encode Data \\ \hline\hline
ShapeWordle~\cite{wang2019shapewordle}  &   -   &     \checkmark        \\
\hline
PAD~\cite{kwan2016pyramid}         &   -   &     -      \\
\hline
ShapeCollage~\cite{shapecollage} &  -    &     -    \\
\hline
Ours & \checkmark & \checkmark 
\end{tabular}
\end{table}
\fi

\paragraph{Qualitative Comparison} 


\begin{figure}[!htb]
  \centering
    \includegraphics[width=1.\linewidth]{fig/compare2.png}
    \caption{Comparison between our method and three existing baselines: yellow areas are the target shape, red areas are where visual objects overlap, and blue areas are where visual objects exceed the target shape.}
  \label{fig:compare}
\end{figure}


\begin{table*}[!htb]
\centering
\caption{\lm{Comparison of the five quality metrics between our method and three baselines on the six examples in Figure~\ref{fig:compare}.}}
\label{table:baseline}
\small 
\begin{tabular}{|c||cc|cc|cc|cc|cc|cc|}
\hline
\multirow{2}{*}{\backslashbox{{Metrics}}{{Methods}}} & \multicolumn{2}{c|}{{Fig.~\ref{fig:compare} Flower}}             & \multicolumn{2}{c|}{{Fig.~\ref{fig:compare} Leaf}}             & \multicolumn{2}{c|}{{Fig.~\ref{fig:compare} Letter P}}              & \multicolumn{2}{c|}{{Fig.~\ref{fig:compare} Australia}}              & \multicolumn{2}{c|}{Fig.~\ref{fig:compare} Moon}             & \multicolumn{2}{c|}{Fig.~\ref{fig:compare} Fish}             \\ \cline{2-13} 
                                  & \multicolumn{1}{c|}{{ShapeW.}} & {Ours} & \multicolumn{1}{c|}{{ShapeW.}} & {Ours} & \multicolumn{1}{c|}{{PAD}} & {Ours} & \multicolumn{1}{c|}{{PAD}} & {Ours} & \multicolumn{1}{c|}{{ShapeC.}} & {Ours} & \multicolumn{1}{c|}{{ShapeC.}} & {Ours} \\ \hline
                                  \hline
                            
{Layout Coverage (LC)}                                & \multicolumn{1}{c|}{0.25}   & 0.28 $\uparrow$     & \multicolumn{1}{c|}{0.18}   &      \textbf{0.29}         & \multicolumn{1}{c|}{\textbf{0.94}}    &    0.80           & \multicolumn{1}{c|}{\textbf{0.91}}             &   0.75            & \multicolumn{1}{c|}{0.67}            &   \textbf{0.86}   & \multicolumn{1}{c|}{0.67}            & \textbf{0.87}     \\ \hline
{Layout Uniformity (LU) $\times 10^{-3}$}                       & \multicolumn{1}{c|}{487.79}            &      {\textbf{80.76 }}         & \multicolumn{1}{c|}{531.95}            &    \textbf{46.44}           & \multicolumn{1}{c|}{\textbf{12.90}}             &    84.25           & \multicolumn{1}{c|}{\textbf{23.43}}             &     118.46          & \multicolumn{1}{c|}{64.77}            &   \textbf{34.56}   & \multicolumn{1}{c|}{50.47}            &    \textbf{21.68}  \\ \hline
{Shape Similarity (SS)}                       & \multicolumn{1}{c|}{2620.64}            &   {\textbf{326.91 }}            & \multicolumn{1}{c|}{2178.15}            &      \textbf{132.39}         & \multicolumn{1}{c|}{\textbf{14.19}}             &     163.98        & \multicolumn{1}{c|}{\textbf{45.12}}             &      309.81        & \multicolumn{1}{c|}{210.66}            & \textbf{67.65}     & \multicolumn{1}{c|}{152.25}            &   \textbf{42.03}   \\ \hline
{Object Overlap (OO) $ \times 10^{-3}$}                       & \multicolumn{1}{c|}{\textbf{0}}            &       {\textbf{0}}        & \multicolumn{1}{c|}{\textbf{0}}            &     0.02          & \multicolumn{1}{c|}{33.83}             &   \textbf{0.14}            & \multicolumn{1}{c|}{55.30}             &       \textbf{0.30}        & \multicolumn{1}{c|}{41.44}            & \textbf{0.09}     & \multicolumn{1}{c|}{40.04}            &    \textbf{0.08}  \\ \hline
{Exceeding Area (EA)$ \times 10^{-3}$}                       & \multicolumn{1}{c|}{\textbf{0}}            &       \textbf{0}        & \multicolumn{1}{c|}{\textbf{0}}            &     \textbf{0}          & \multicolumn{1}{c|}{7.17}             &     \textbf{0}          & \multicolumn{1}{c|}{21.84}             &      \textbf{0}         & \multicolumn{1}{c|}{18.31}            &   \textbf{0}   & \multicolumn{1}{c|}{7.86}            &  \textbf{0}    \\ \hline
\end{tabular}
\end{table*}

\paragraph{Quantitative Comparison} We compared our method with the other three over five metrics. We tested ShapeWordle and our method on two target shapes (`flower' and `leaf' in Figure~\ref{fig:compare}) from the ShapeWordle website~\footnote{https://www.shapewordle.com/}. PAD and our method were tested using two examples from the PAD work~\cite{kwan2016pyramid} (`Australia' and `Letter P'). For comparison with ShapeImage, two general target shapes were chosen, `Moon' and `Fish'. Table~\ref{table:baseline} summarizes the five metrics of different methods across the six examples. 

Figure~\ref{fig:compare} visualizes the collage results, where the target shapes are colored in yellow, and visual objects are colored in gray. To highlight the overlaps, the overlaps among visual objects (OO) are colored in red, and areas exceeding the target shapes (EA) are colored in blue. As can be seen, compared to ShapeWordle, our method consistently demonstrates superior performance in Layout Coverage (LC), Layout Uniformity (LU), and Shape Similarity (SS). In both the `leaf' and `flower' examples, our method has much less space left, and the distribution is more even. Our method outperformed ShapeImage in all five metrics. As can be seen in the `Moon' and `Fish' examples, our method achieves larger coverage, but with much more even distribution, less overlap among objects, and less exceeding from the target shapes. As shown in the `Australia' and `Letter P' examples, PAD gets a more compact layout than ours, with less space left, which results in better scores in Layout Coverage, Layout Uniformity, and Shape Similarity. However, PAD causes more severe overlapping (i.e., the red and blue areas in Figure~\ref{fig:compare}) than ours.

\paragraph{Time Cost Comparison} In terms of time cost, ShapeWordle and ShapeCollage complete a collage in a matter of seconds. Our method takes approximately one minute on average, while PAD requires the longest time, taking around 30 minutes to complete a single example. In Figure~\ref{fig:pad}(top), it takes over 700 minutes to arrange 1225 graphical items in PAD, while it only costs \lmn{?} seconds for our method. 

\begin{figure}[!htb]
  \centering
    \includegraphics[width=1.\linewidth]{fig/time_pad_min.png}
    \caption{Time cost of our method and others: (top) with PAD~\cite{kwan2016pyramid}, and (bottom) with Minkowski Penalty~\cite{minarvcik2024minkowski}.}
  \label{fig:pad}
\end{figure}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}


% \subsection{Computation Efficiency}
% \label{subsec:comp_eff}

\iffalse
To assess the computational consumption of our method, we conducted a performance evaluation with two experimental variables, i.e., \textit{primitive scale} (i.e., the number of visual primitives) and \textit{primitive complexity} (i.e., the number of cubic Bézier curves to represent one visual primitive). The primitive scale was studied in five levels (i.e.,  50, 100, 200, 400, and 800.) Primitive complexity was studied in \lm{three} levels, i.e., \lm{10, 20, and 40} for low, middle, and high complexity respectively. There are 15 conditions in total (5 primitive scales x 3 primitive complexities). For each condition, our method was tested in \lm{a general target shape ('bird' as shown in Figure~\ref{fig:sdf}). \lm{Visual primitives in all testing are initialized by the SDF method.} The \textit{average time cost per epoch} and \textit{the number of epochs needed to achieve convergence} to an overall low loss was reported.}

\paragraph{\textbf{Time Cost}} The time cost per epoch in different conditions of primitive complexities and primitive scales are shown in Figure~\ref{fig:time_converage}(a), with the following findings: (1) \textit{Effect of primitive scale:} As the number of visual primitives increases, the average time cost per epoch increases in a near-linear trend, demonstrating the algorithm’s efficient scalability and its ability to handle larger datasets without a significant drop in performance. (2) \textit{Effect of primitive complexity:} Comparing the low, middle, and high primitive complexities, there is no significant difference in the time cost per epoch among the three levels. This suggests that the computational efficiency remains consistent regardless of the number of Bézier curves used to represent a visual primitive. 

% (3) \textit{Scalability:} our method demonstrates good scalability as the number of primitives increases. Despite the increase in time cost per epoch, the time cost per epoch remains within a reasonable range, indicating that the method can handle larger scenes with a manageable increase in computational resources.

%Overall, although the average time cost per epoch increases with the arise of primitive scale and complexity, our method demonstrates scalability without a significant increase in time cost per epoch.

%\dc{There is a bit of redundancy in the above two sentences}\lmc{agree, I revised it.}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}

% \begin{table}[]
% \centering
% \small
% \begin{tabular}{c|cc|c}
% \hline
%                                             & \multicolumn{2}{c|}{\textbf{Primitive Complexity}}                               &                                                                                                    \\ \cline{2-3}
% \multirow{-2}{*}{\textbf{\# of Primitives #}} & \multicolumn{1}{c|}{\textbf{Low (s)}}             & \textbf{High (s)}           & \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Avg. \\ Time Cost per Epoch (s)\end{tabular}}} \\ \hline\hline
% 50                                          & \multicolumn{1}{c|}{0.42} & 0.71 & 0.56                                                                       \\ \hline
% 100                                         & \multicolumn{1}{c|}{0.66} & 1.39 & 1.02                                                                       \\ \hline
% 200                                         & \multicolumn{1}{c|}{1.14} & 2.32 & 1.73                                                                       \\ \hline
% 400                                         & \multicolumn{1}{c|}{2.68} & 3.69 & 3.19                                                                       \\ \hline
% 600                                         & \multicolumn{1}{c|}{3.99} & 4.68 & 4.34                                                                       \\ \hline
% 800                                         & \multicolumn{1}{c|}{5.02} & 5.34 & 5.18                                                                       \\ \hline
% 1000                                        & \multicolumn{1}{c|}{5.68} & 5.83 & 5.75                                                                       \\ \hline
% \end{tabular}
% \caption{Average time cost per epoch for different numbers of primitives and complexity levels.}
% \label{table:timecost}
% \end{table}

% \begin{table}[]
% \centering
% \small
% \begin{tabular}{c|cc|c}
% \hline
%                                             & \multicolumn{2}{c|}{\textbf{Primitive Complexity}}                               &                                                                                                    \\ \cline{2-4}
% \multirow{-2}{*}{\textbf{\# of Primitives }} & \multicolumn{1}{c|}{\textbf{Low (s)}}             & \textbf{High (s)}           & \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Avg. \\ Time Cost per Epoch (s)\end{tabular}}} \\ \hline\hline
% 50                                          & \multicolumn{1}{c|}{0.42} & 0.71 & 0.56                                                                       \\ \hline
% 100                                         & \multicolumn{1}{c|}{0.66} & 1.39 & 1.02                                                                       \\ \hline
% 200                                         & \multicolumn{1}{c|}{1.14} & 2.32 & 1.73                                                                       \\ \hline
% 400                                         & \multicolumn{1}{c|}{2.68} & 3.69 & 3.19                                                                       \\ \hline
% 600                                         & \multicolumn{1}{c|}{3.99} & 4.68 & 4.34                                                                       \\ \hline
% 800                                         & \multicolumn{1}{c|}{5.02} & 5.34 & 5.18                                                                       \\ \hline
% 1000                                        & \multicolumn{1}{c|}{5.68} & 5.83 & 5.75                                                                       \\ \hline
% \end{tabular}
% \caption{Average time cost per epoch for different numbers of primitives and complexity levels.}
% \label{table:timecost}
% \end{table}



% % \usepackage{multirow}
% \begin{table}
% \small
% \centering
% \begin{tabular}{|c|c|c|c|c|} 
% \hline
% \multirow{2}{*}{\textbf{\# of Primitives}} & \multicolumn{3}{c|}{\textbf{Curve Segments}}  & \multirow{2}{*}{\textbf{Avg.}}  \\ 
% \cline{2-4}
%                                            & \textbf{10} & \textbf{20} & \textbf{40} &                                 \\ 
% \hline
% 50                                         & 0.48            & 0.53            & 0.57            & 0.56                            \\ 
% \hline
% 100                                        & 0.57            & 0.58            & 0.57            & 0.57                            \\ 
% \hline
% 200                                        & 0.67            & 0.67            & 0.67            & 0.67                            \\ 
% \hline
% 400                                        & 0.85            & 0.92            & 0.9             & 0.89                            \\
% \hline
% 800                                        & 0.85            & 0.92            & 0.9             & 0.89                            \\
% \hline
% \end{tabular}
% \caption{Average time cost per epoch for different numbers of primitives and complexity levels.}
% \label{table:timecost}
% \end{table}



\paragraph{\textbf{Convergence}} Figure~\ref{fig:time_converage}(b) shows the MSE loss over iterations of the 15 conditions of primitives scales and complexity levels. As can be seen, our method can quickly converge in a closed target shape with the SDF-based initialization around 100 epochs. With the average time cost per epoch from 0.45s to 0.8s, the total time consumed for a general collage optimization can be estimated up to 1.5 minutes (with 800 visual primitives). 

As above, we evaluated the general computation efficiency of our method under the 15 conditions of primitive scales and primitive complexities, with the SDF initialization method. It is important to note that complex target shapes and different primitive initialization methods have the potential to introduce variations in the convergence epochs, therefore the time cost. Table~\ref{tab:example} provides the information of some examples generated in Figure~\ref{fig:gallery}. \lm{As seen here, using the SDF-based position initialization, our collage technique converges faster than the MAT-based method initialization in most of the examples. Also, it is important to acknowledge the need for further investigation into the specific impact of primitive complexity on convergence epochs. For example in Figure~\ref{fig:gallery}(a), it took similar rounds to converge for both two initialization.} %\lmc{to be checked}

\begin{figure}[!htb]
  \centering
    \includegraphics[width=1.\linewidth]{fig/performance8.png}
    % {img/match.png}
    \caption{Time cost and convergence: (a) average time cost per epoch for different primitive scales (x-axis) and complexity levels (blue, green, and red); (b) MSE loss values changing over iterations.}
  \label{fig:time_converage}
\end{figure}

% \begin{figure}[!htb]
%   \centering
%     \includegraphics[width=1.\linewidth]{fig/iteraion2.png}
%     % {img/match.png}
%     \caption{MSE loss values changing over iterations \lmc{add the curves using SDF initialization.}}
%   \label{fig:converge}
% \end{figure}

%\dc{Again, I think the cost is a function of the number of control point... it is the cost of the differential renderer operation} 
%\lmc{yes, cost per epoch is a function of control points, here I mis-attributed it to the fitting boundaries... I have revised it. }

\begin{table}[!htb]
\caption{Time cost for examples in Figure~\ref{fig:gallery}.}
\label{tab:example}
\scriptsize
\begin{tabular}{c|c|c|cc|cc}
\hline
\multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Examples}}} & \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\# of\\Primi.\end{tabular}}}} & \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Time Cost\\ per Epoch (s)\end{tabular}}}} & \multicolumn{2}{c}{\lm{SDF Init.}}                                                                                                                          & \multicolumn{2}{c}{\lm{MAT Init.}}                                                                                                                          \\ \cline{4-7} 
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{\textbf{\lm{\begin{tabular}[c]{@{}c@{}}Cov. \\ Epoch\end{tabular}}}} & \multicolumn{1}{c|}{\textbf{\lm{\begin{tabular}[c]{@{}c@{}}Time \\Cost (s)\end{tabular}}}} & \multicolumn{1}{c|}{\lm{\begin{tabular}[c]{@{}c@{}}Cov. \\Epoch\end{tabular}}} & \multicolumn{1}{c}{\lm{\begin{tabular}[c]{@{}c@{}}Time \\Cost (s)\end{tabular}}} \\ \hline \hline
Fig. 7(a)                                       & 72                                                                                               & 0.30                                                                                                      & \multicolumn{1}{l|}{600}                                   & 180.8                                                                          & \multicolumn{1}{l|}{600}                                                    &            179.8                                                                  \\ \hline
Fig. 7(b)                                       & 105                                                                                               & 0.28                                                                                                    & \multicolumn{1}{l|}{150}                                                       & 49.6                                                                           & \multicolumn{1}{l|}{400}                                                          &                    105.7                                                          \\ \hline
Fig. 7(e)                                       & 80                                                                                               & 0.36                                                                                                      & \multicolumn{1}{l|}{250}                                                       & 93.9                                                                          & \multicolumn{1}{l|}{500}                                                          &                     178.1                                                         \\ \hline
\lm{Fig. 7(f)}                                       & 216                                                                                               & 0.40                                                                                                    & \multicolumn{1}{l|}{150}                                                       & 68.8                                                                         & \multicolumn{1}{l|}{300}                                                          &         110.5                                                                     \\ \hline
\lm{Fig. 7(g)}                                       & 252                                                                                               & 0.49                                                                                                    & \multicolumn{1}{l|}{120}                                                       & 69.4                                                                         & \multicolumn{1}{l|}{250}                                                          &    112.5                                                                          \\ \hline
\end{tabular}
\end{table}

\fi

% \paragraph{\lm{Predictive Feedback}}

% \lmc{here we introduce a design for users to predict the result of collage, and ask people to vote for its prediction-ability, report it.} 


% \subsection{Data Encoding Feasibility}
% \label{subsec:visualquality}

% As introduced in Section~\ref{subsec:loss}, there is no data encoding loss if the scale of all visual primitives is uniform, namely a global scale to all visual primitives. In this section, we report the results of evaluating our methods based on data encoding fidelity, when primitives are scaled individually and constrained by the data fidelity loss. 

% Figure~\ref{fig:fidelity} illustrates the change in data fidelity loss over iterations. On average, the convergence of the loss occurs around 350 epochs, regardless of the number of primitives. As the number of primitives increases, there is a slight increase in the data fidelity loss. This observation can be attributed to the increased difficulty in maintaining correspondence between a larger number of primitives and the raw data. 

% \begin{figure}[!htb]
%   \centering
%     \includegraphics[width=1.\linewidth]{fig/fidelity.jpg}
%     % {img/match.png}
%     \caption{Data fidelity loss changing over iterations}
%   \label{fig:fidelity}
% \end{figure}

% We tested on different weight $\gamma$ of data fidelity loss in the optimization, results in different encoding errors. Here, the encoding errors is computed as the average corresponding difference between every pair of data items in the visualization. A clear negative correlation between the weight and loss can be observed: with a small weight (=$1e5$ in our study), the encoding error can be around $\pm 3.0\%$, with a larger weight (=$1e8$), the encoding error can be reduced to $\pm 0.4\%$. 

% %0.03285448574950895, 0.018529358566932018, 0.005325827505275337, 0.004776429812089888

% % \begin{figure}[!htb]
% %   \centering
% %     \includegraphics[width=.95\linewidth]{fig/fi_weight.png}
% %     % {img/match.png}
% %     \caption{The relationship between data encoding error and the weight of data fidelity. \lmc{to be updated}}
% %   \label{fig:fi_weight}
% % \end{figure}

% Our framework offers customization options to cater to different requirements on data fidelity. When dealing with visualizations that demand high encoding precision, such as a Square Map depicting 100 companies in the USA (left-top one in Figure~\ref{fig:teaser}), we have two approaches. One is, we can employ a global scale transformation on the primitives to ensure accurate representation. Alternatively, we can employ individual scale transformation, and constrain the optimization problem by assigning a large weight to the data fidelity loss term. This weight emphasizes the importance of preserving the fidelity of the underlying data during the optimization process.

% Conversely, if a visualization has a more relaxed requirement on data encoding precision, we can assign a smaller weight to the data fidelity loss. This flexibility allows to strike a balance between fidelity and other optimization objectives. However, it is important to note that a large weight on the fidelity loss may negatively impact the optimization of the other two losses, namely the smoothness and boundary losses. For instance, in the case of USA map visualization, applying a large weight to the data fidelity loss might result in overlapping rectangles. 


%By providing the ability to customize the weight of the data fidelity loss, our framework enables users to fine-tune the trade-off between fidelity and other optimization objectives based on their specific visualization requirements.


==> tex/terminology.tex <==
# Object-space: 
# Image-space: 
